A Survey of Unikernel Security: Insights and Trends from a Quantitative Analysis

Unikernels, an evolution of LibOSs, are emerging as a virtualization technology to rival those currently used by cloud providers. Unikernels combine the user and kernel space into one "uni"fied memory space and omit functionality that is not necessary for its application to run, thus drastically reducing the required resources. The removed functionality however is far-reaching and includes components that have become common security technologies such as Address Space Layout Randomization (ASLR), Data Execution Prevention (DEP), and Non-executable bits (NX bits). This raises questions about the real-world security of unikernels. This research presents a quantitative methodology using TF-IDF to analyze the focus of security discussions within unikernel research literature. Based on a corpus of 33 unikernel-related papers spanning 2013-2023, our analysis found that Memory Protection Extensions and Data Execution Prevention were the least frequently occurring topics, while SGX was the most frequent topic. The findings quantify priorities and assumptions in unikernel security research, bringing to light potential risks from underexplored attack surfaces. The quantitative approach is broadly applicable for revealing trends and gaps in niche security domains.

==> content/Background.tex <==
\subsection{VMs and Containers}
Virtual Machines and containers differ in how they interact with the host and its kernel. Since each VM is a full OS with its own kernel, they need more specialized access to the host environment. VMs utilize a hypervisor, or Virtual Machine Monitor, which exists between the VM and the host OS and acts as an intermediary for system calls and resource management \cite{SecuritySurvey, Virt_IssuesAndSolutions, CompVirtandCont}. This required middleman provides separation between the VM and the host OS, and while it does introduce more complexity it also provides greater independence to the VM \cite{SecuritySurvey, Virt_IssuesAndSolutions}. Special hardware extensions are required to enable virtualization capabilities \cite{SecuritySurvey}, and while most modern hardware platforms possess these they are generally not enabled by default on consumer devices.

Compared to VMs, containers do not have the same hardware requirements as VMs. Container technology such as Docker is a user space application and does not utilize a hypervisor to interact with the host OS \cite{SecuritySurvey, CompVirtandCont}. Instead, the application is used to manage all the necessary resources requests and interactions with the host kernel \cite{SecuritySurvey, CompVirtandCont}. Container technology depends on the host kernel to support several technologies in order to achieve its functionality \cite{SecuritySurvey}. On Linux systems two of these are cgroups and namespaces, which provide the isolation and permission mechanisms for containers \cite{Virt_IssuesAndSolutions}.

Containers offer an advantage over VMs in that their base image is smaller, however containers have a reduced feature set compared to VMs \cite{CompVirtandCont}. While this sounds like a disadvantage for containers, removing unnecessary or unused features provides more space for additional containers to run. Where only one VM could exist before, now dozens of containers can run different applications concurrently, but isolated from each other \cite{CompVirtandCont, Virt_IssuesAndSolutions}. This last component is very important in cloud infrastructures where different containers execute on the same hardware, but must be isolated from others for best security practices \cite{CompVirtandCont, Virt_IssuesAndSolutions}.

VMs initial rise to prominence was due in large part to their customization and flexibility \cite{Disco}. Tasks that would previously require multiple dedicated devices could now be run on one physical machine with multiple VMs \cite{Disco, SecuritySurvey}. This capability in the early 1990s and even into the 2000s was extremely effective; until the Internet \cite{CloudCyberSecurity}. The explosion of the Internet required data centers do grow rapidly, and where the full capabilities of VMs used to be needed now much slimmer technologies provided greater benefit \cite{CloudCyberSecurity, VMSurvey}. Container technology such as Docker and LXC provide an advantage due to their reduced space and execution requirements \cite{CompVirtandCont, VMSurvey}. By eliminating extra components, such as graphical interfaces and individual kernels, the resources required by containers are drastically reduced \cite{SecuritySurvey}. However as the Internet continued to expand the need for more space efficient virtualization only continued to rise \cite{CloudCyberSecurity, Unikernel:LibOSForTheCloud, RethinkingLibOS}.

\subsection{Unikernels}
Unikernels are an evolution of an old idea: Library Operating Systems (LibOS.) The origins of LibOSs stem from the early 1990s \cite{RethinkingLibOS}. The principle idea being OS functionality is implemented in the form of libraries, which are customized to increase performance of the application by giving it closer access to hardware \cite{RethinkingLibOS}. However, the rise of Virtual Machines (VMs) around the same time quickly overshadowed LibOSs \cite{Disco} as a virtualization technique. Virtual Machine's ability to replicate the entire OS and run applications, compared to the customization required to enable LibOSs to run \cite{RethinkingLibOS}, put LibOSs at a disadvantage. Additionally VMs provided a way for several OSs to run on one physical device \cite{Virt_IssuesAndSolutions}. Several decades later, after the flourishing of technological advances like the Internet, LibOSs reimerged as unikernels. \cite{Unikernel:LibOSForTheCloud}.

Unikernels are different from VMs and containers in several key ways. Unikernels, as the name implies, ``uni''fy the user and kernel address spaces into one \cite{Unikernel:LibOSForTheCloud,UnikernelApproachCloud}. This also means when the unikernel is compiled, all necessary kernel functionality along with the application code are combined into one unified binary \cite{Unikernel:LibOSForTheCloud,FreshLookAtIsolationPlatforms}. Combining the application and kernel into one binary does come with some benefits. Utilizing syscalls to invoke kernel functionality and context switches into and out of kernel are no longer required, and simpler function call implementations can be used instead \cite{Unikernel:LibOSForTheCloud, RethinkingLibOS, unikernelIsolation_MPK}. The direct invocation of kernel code in this way is where the tradition of LibOSs shines through.

Furthermore, unikernels have a drastically smaller memory requirement than other virtualization techniques \cite{Unikernel:LibOSForTheCloud, FreshLookAtIsolationPlatforms}. Unikernels achieve this through a build system specifically designed to compile in only the necessary components required to execute the unikernel's application \cite{UnikernelApproachCloud, Unikernel:LibOSForTheCloud}. In contrast, if a Linux VM is built to host a web server, that VM is built with all the core Linux utilities and libraries in addition to any that are required by the web server. Even containers, while not comprising the entire OS, still possess a plethora of functionality above and beyond its intended function. The lack of additional functionality is what most papers cite as a security benefit \cite{CloudCyberSecurity, UnikernelSecurityPerspective}, however there are a few that provide an opposing view \cite{michaels2019assessing}.

To achieve the reduced size, many familiar core security features are removed: Address Space Layout Randomization (ASLR), Non-executable Bits (NX), stack canaries, etc \cite{michaels2019assessing, Unikernel:LibOSForTheCloud, UnikernelSecurityPerspective}. Adhering to the core reductionist principle adopted by unikernels, these features have been removed to save space, simplify the code base, and eliminate extra, unnecessary features \cite{Unikernel:LibOSForTheCloud, michaels2019assessing, UnikernelSecurityPerspective}. Typically papers do not refer to this removal as a security problem, as the typical attack paths that utilize ``bash'' or ``sh'' do not exist as those tools are not built into the unikernel by default \cite{UnikernelSecurityPerspective, michaels2019assessing}.

The development and construction of unikernels is the primary focus of research papers on unikernels, with some focusing on processor specific security implementations \cite{Uniguard, unikernelIsolation_MPK} and others discussing security more broadly \cite{CloudCyberSecurity, UnikernelSecurityPerspective}. While collecting papers for the research corpus, only one paper was found to provide a comprehensive analysis of unikernel security \cite{michaels2019assessing}. While its findings do showcase vulnerabilities that existing security techniques are designed to fix \cite{michaels2019assessing}, their removal in unikernels means these vulnerabilities could pose a significant problem once again.


==> content/Cut.tex <==

Unikernels, an evolution of LibOSs, are emerging as a virtualization
technology to rival those currently used by cloud
providers. Unikernels combine the user and kernel space into one
``uni''fied memory space and omit functionality that is not necessary
for its application to run, reducing the resources each unikernel
requires drastically. The removed functionality is far-reaching and
includes what have become common place security technologies such as
ASLR, DEP, and NX-bits.
%any transition here mentioning investigating possible impacts or that the impacts of such choices are not yet know... and to say perhaps that this research is an effort toward that goal?
%is the following specific enough?

